MTRNet: A Generic Scene Text Eraser

Text removal algorithms have been proposed for uni-lingual scripts with regular shapes and layouts. However, to the best of our knowledge, a generic text removal method which is able to remove all or user-specified text regions regardless of font, script, language or shape is not available. Developing such a generic text eraser for real scenes is a challenging task, since it inherits all the challenges of multi-lingual and curved text detection and inpainting. To fill this gap, we propose a mask-based text removal network (MTRNet). MTRNet is a conditional adversarial generative network (cGAN) with an auxiliary mask. The introduced auxiliary mask not only makes the cGAN a generic text eraser, but also enables stable training and early convergence on a challenging large-scale synthetic dataset, initially proposed for text detection in real scenes. What's more, MTRNet achieves state-of-the-art results on several real-world datasets including ICDAR 2013, ICDAR 2017 MLT, and CTW1500, without being explicitly trained on this data, outperforming previous state-of-the-art methods trained directly on these datasets.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:con}
In this study, we propose a generic scene text eraser, MTRNet. It addresses the lack of a generic method for text removal from all kinds of scenes with all kinds of text. In this work, MTRNet is trained on a synthetic text detection dataset, and it surpasses previous studies trained on real scene datasets for several benchmark datasets. MTRNet achieves this by appending text masks with the input image prior to passing the input to a cGAN. Text masks not only improve the results of the cGAN, but also make the training of the cGAN on a challenging synthetic dataset more stable and efficient.

%Text removal methods automatically remove texts in scenes. It is a very useful application for image restoration, privacy protection, and even image retrieval. It has been closely connected with two challenging tasks: \textit{text detection} and \textit{inpainting} till recent studies solve it as image translation with deep convolutional neural networks (CNN). Although their results are new state-of-the-art, lack of generalization and partial removing is the bottleneck. To overcome these, we proposed a mask-based text removal approach, which has better generalization and robust partial removing capability via selecting text masks. Our method has achieved new state-of-the-art quantitative and qualitative results.

\section{Acknowledgement}
This research was supported by an Advance Queensland Research Fellowship Award.

==> method.tex <==
\section{Method}
\label{sec:met}

\begin{figure*}[t!]
	\includegraphics[width=\textwidth]{images/maskdiag}
	\caption{The overall structure of  MTRNet. It is composed of a generator and discriminator. The input to the generator is a concatenation of the input image and its text mask, and the input to the discriminator is a concatenation of the groundtruth/generator output and the input of the generator.}
	\label{fig:model}
\end{figure*}
\noindent
{\bfseries{Conditional generative adversarial networks (cGAN)}} constitute a framework which can be adapted for image-to-image translation \cite{isola2017image}. They are composed of a Generator ($G$) and a Discriminator ($D$). In an image-to-image transformation task, every pixel in an image is mapped from the original domain to the target domain. $G$ is trained to learn the mapping, while $D$ is used to evaluate the performance of $G$. The cGAN is trained with pairs of corresponding images ${(x, y)}$, where $x, y$ belongs to source and target domains respectively. The following objective loss is applied for training,

\begin{equation}
G^*=arg\min_{G}\max_{D}\mathcal{L}_{cGAN}(G,D) + \lambda \mathcal{L}_{L1}(G), 
\end{equation}

where $\mathcal{L}_{cGAN}(G,D)$ is the adversarial loss given in Eq. \ref{eq:gan}, and $\mathcal{L}_{L1}$ is the L1 loss given in Eq. \ref{eq:l1}. Here, the L1 loss is guiding the model to produce outputs which have the same general structure as the ground truth, while the adversarial loss teaches the model to approximate the distribution of the high-frequency signals that appear in the ground truth,

\begin{multline}
\mathcal{L}_{cGAN}= \min_{G}\max_{D}\mathbb{E}_{x,y \sim p_{data}(x,y)}[logD(x,y)]+ \\
\mathbb{E}_{x \sim p_{data}(x)}[log(1 - D(x, G(x))],
\label{eq:gan}
\end{multline}

\begin{equation}
\mathcal{L}_{L1}(G)=\mathbb{E}_{x,y\sim p_{data(x,y)}}[\left \|  y-G(x) \right \|_1].
\label{eq:l1}
\end{equation}

The cGAN provides an intuitively appealing solution for text removal as the latter is also an image transformation problem. However, due to the fact that text is sparse in real-life scenes, the source and target domain are very similar. The similarity between source and target domain is one of the reasons as to why training cGANs with real scene datasets is challenging. What's more, even a well-trained cGAN has a limited applicable scope.
%What's more, partial and universal text removal is also not supported by cGAN. 

In this study, the text mask of the input is employed to solve the aforementioned disadvantages of cGANs. The text mask of the input is sent to both G and D as an extra channel of the input. In other words, we replace $x$ with $(x, f(x))$, where $f$ is a function for generating text masks for $x$, which can be a text detection algorithm or manual input. During training, it boosts the convergence of both $G$, and $D$, while at inference it endows a generic and partial text removal ability to the model. 

The overall structure of MTRNet is given in Fig. \ref{fig:model}. It is composed of a G and a D, which are introduced in detail in the following sections.
\\[1.5ex]
\noindent
{\bfseries{Generator:}} In this work, U-Net \cite{ronneberger2015u} is the backbone of G. U-Net is a skip-connected fully convolutional neural (FCN) network. It is composed of an encoder and a decoder, which share convolutional channels. Those shared convolutional channels share information from the encoder to the decoder, providing useful context information for generating realistic images. U-Net receives an input of size $256 \times 256 \times 4$, which is a concatenation of red, green and blue channels of an image and the corresponding text-mask. All images and their corresponding masks are resized to 256 square while retaining the original aspect ratio though zero padding. The input is normalized to the range [-1, 1]. 

The encoder is composed of seven convolutional layers with kernel size 4, stride step 2, and zero padding. The number of kernels are $64, 128, 256, 512, 512, 512, 512$. LeakyReLU and batch normalization are applied in all Convolutional layers.

The decoder is composed of seven deconvolution layers with stride step 2 and eight convolutional layers with stride step 1. Deconvolution layers are applied to enlarge the size of the input of the decoder to the size of original image. The output of each deconvolution layer is sent to a subsequent convolutional layer, which stacks the output of the corresponding convolutional layer in the encoder. All layers have kernels with size 4, and zero padding. As with the encoder, batch normalization and LeakyRelu are applied to all layers except the last convolutional layer where a tanh function is used to map the output to the range [-1, 1].
%Outputs of first six deconvolutional layers are stacked with the output of the corresponding convolutional layer of the encoder, and sent to the next convolutional convolutional layer. The number of kernel of first three deconvolution and convolutional layers is 512, while it is divided by half in each deconvolution layer till reach to 64.
%
%\oc{L1 loss is applied with a weight of 100.}
%
%batch normalization
%first layer batch normalization
%leaky relu
%linear transform layer
\\[1.5ex]
\noindent
{\bfseries{Discriminator:}}
%batch normalization
%and a fully convolutional neural network as backbone of discriminator. The network outline is displayed in Figure \ref{fig:model}.
%The discriminator is a fully convolutional neural network (FCN). 
%The mask is also applied in discriminator. The input of discriminator is stack of mask, input, and output of generator or the ground truth. For discriminator, a patch-based loss is proposed in Pix2Pix. In our work, patch-based loss is applied in pixel level. Therefore, a fully convolutional neural (FCN) is applied in this work. It is also composed of encoder and decoder part. The encoder is composed four convolutional layer, and decoder is composed of four deconvolutional layer and one convolutional layer.
The discriminator architecture follows PatchGAN \cite{isola2017image}, which is designed to penalize the structure of the input (real image or generator output) at the scale of patches. It classifies if each patch as real or fake. In this work, the patch size of D is set to $1 \times 1$. Although a big patch size is beneficial for efficiency, the discriminator fails to focus on the text removal task because of the sparsity of text in a scene. With pixel-level patches, losses at text masks are back propagated to the model sufficiently.

A FCN is used as the backbone for D. Its output size is set to the same size as the input to get pixel level patches. As shown in Fig. \ref{fig:model}, it is composed of an encoder and a decoder. The encoder has four convolutional layers, while the decoder has four deconvolutional layers and one convolutional layer. In the encoder, the number of kernels are $64, 128, 256, 512$, while in the decoder, the number of kernels are $512, 256, 128, 64, 1$. All convolutional and deconvolutional layers except the last convolutional layer have kernels with the size of $4$, and a step stride of 2. They are also activated by LeakyRelu, and batch normalized. However, no activation and normalization are applied to the last convolutional layer. Its stride size is set to 1. Note zero padding is applied to all layers.
\\[1.5ex]
\noindent
{\bfseries{Training:}}
We have implemented our model with and without the mask using TensorFlow. Adam is chosen as the optimizer and its momentum is set to 0.9. The initial learning rate is 0.0002, and decays by a factor 0.95 after every 2 epochs. The size of an epoch is 3,125 iterations. The batch size is set to 16. The model is trained for 96 epochs.
%Each batch takes approximately 2s on a NVIDIA Tesla GeForce GTX 1080 Ti GPU and in total the model takes about 144 hours to converge.
